The LDBC Social Network Benchmark Interactive workload v2: A transactional graph query benchmark with deep delete operations

The LDBC Social Network Benchmark's Interactive workload captures an OLTP scenario operating on a correlated social network graph. It consists of complex graph queries executed concurrently with a stream of updates operation. Since its initial release in 2015, the Interactive workload has become the de facto industry standard for benchmarking transactional graph data management systems. As graph systems have matured and the community's understanding of graph processing features has evolved, we initiated the renewal of this benchmark. This paper describes the draft Interactive v2 workload with several new features: delete operations, a cheapest path-finding query, support for larger data sets, and a novel temporal parameter curation algorithm that ensures stable runtimes for path queries.

==> tab-operations.tex <==
\begin{table}[htb]
    \vspace{-3ex}
    \centering
    \setlength\tabcolsep{4pt}
    \begin{tabular}{@{}lrlr@{}}
        \toprule
        \thead{Operation type} &
        \thead{\#}             &
        \thead{Complexity}     &
        \thead{Runtime (ms)}
        \\
        \midrule
        Complex read           & 14 & $\mathcal{O}(d^3 \log n)$, $\mathcal{O}(n+e)$, $\mathcal{O}(n \log n + e)$ & $1 \ldots 500$               \\
        Short read             & 7  & $\mathcal{O}(\log n)$                                                      & $0.1 \ldots 75$              \\
        Insert                 & 8  & $\mathcal{O}(\log n)$                                                      & $0.1 \ldots 100$             \\
        Delete                 & 8  & \emph{varies}                                                              & $1 \ldots 300$ \\
        \bottomrule
    \end{tabular}
    \caption{
        Theoretial complexity and runtime of the operations in the workload.
    }
    \label{tab:operations}
    \vspace{-4.5ex}
\end{table}


==> tab-related-work.tex <==
\begin{table}[htb]
    \centering
    \setlength\tabcolsep{2pt}
    \footnotesize
    \begin{tabular}{@{}l|l|r|c|cc|ll@{}}
        \toprule
        \theadbar{Benchmark}                                         &
        \theadbar{Distinguishing features}                           &
        \theadbar{Scale}                                             &
        \theadsidebar{\#Ops}                                         &
        \theadside{Inserts}                                          &
        \theadsidebar{Deletes}                                       &
        \theadsideleft{Required}{isolation}                                                                                                                      \\
        \midrule
        LDBC SNB Interactive v2                                      & transactional graph queries & \numprint{30000}      & 37 & \yes & \yes   & \textsf{SI}    \\
        LDBC FinBench                                                & strict latency guarantees   & \myast~\numprint{100} & 34 & \yes & \yes   & \textsf{RC}    \\
        \midrule
        TPC-C~\cite{tpcc}                                            & complex transactional mix   & \numprint{4928000}    & 5  & \yes & \maybe & \textsf{RR}    \\
        TPC-H~\cite{tpch}                                            & complex analytical mix      & \numprint{100000}     & 22 & \yes & \maybe & \textsf{RC} ?! \\
        \midrule
        \bottomrule
    \end{tabular}
    \caption{
        Comparison of related benchmarks.
        \emph{Scale:} size of the largest data set measured in textual format.
        For TPC benchmarks, we indicate the largest audited size.
        \emph{Isolation levels:}
        \textsf{RC}: read committed,
        \textsf{RR}: repeatable read,
        \textsf{SI}: snapshot isolation.
        Legend:
        \yes~yes,
        \no~no,
        \maybe~only simple delete operations are included,
        \myast~later versions will support larger scale factors.
    }
    \label{tab:benchmark-characteristics}
\end{table}

\todo{does TPC-C really require RR?}

\todo{what is the minimum isolation level required by TPC-H?}



==> tab-snb-workloads.tex <==
\begin{table}[htb]
    \vspace{-2.5ex}
    \centering
    \footnotesize
    \setlength\tabcolsep{2.2pt}
    \begin{tabular}{@{}llclcl@{}}
        \toprule
        \textbf{Workload}
                                                    &
        \multicolumn{1}{c}{\textbf{Interactive~v1}} &                &
        \multicolumn{1}{c}{\textbf{Interactive~v2}} &                &
        \multicolumn{1}{c}{\textbf{BI}}
        \\ \midrule
        Release year                                & 2015           &               & 2023               &              & 2022
        \\ \midrule
        Target metrics                              & throughput     & $\Rightarrow$ & throughput         &              & throughput, power     \\
        Largest scale factor                        & SF\OneK        &               & SF\ThirtyK         & $\Leftarrow$ & SF\ThirtyK            \\
        Update types                                & inserts        &               & inserts, deletes   & $\Leftarrow$ & inserts, deletes      \\
        Update frequency                            & continuous     & $\Rightarrow$ & continuous         &              & daily batches         \\
        Concurrent updates                          & required       & $\Rightarrow$ & required           &              & optional              \\
        Required isolation level                    & read committed &               & snapshot isolation & $\Leftarrow$ & snapshot isol.~\myast \\
        \midrule
        Read query footprint                        & small          & $\Rightarrow$ & small              &              & large                 \\
        Cyclic joins                                & no             & $\Rightarrow$ & no                 &              & yes                   \\
        Cheapest path queries                       & no             &               & yes                & $\Leftarrow$ & yes                   \\
        Query variants                              & no             &               & yes                & $\Leftarrow$ & yes                   \\
        \midrule
        General-purpose lang's                      & allowed        & $\Rightarrow$ & allowed            &              & not allowed           \\
        Driver runtime                              & Java 8         & $\Rightarrow$ & Java 17            &              & Python 3              \\
        \bottomrule
    \end{tabular}
    \caption{
        Comparison of the LDBC Social Network Benchmark's workloads.
        Arrows ($\Rightarrow$/$\Leftarrow$) denote influences between the workloads, showing that \interactivevtwo mostly builds on \interactivevone but is also heavily influenced by the \biw.
        Legend:
        \myast~snapshot isolation is required if concurrent updates are used.
    }
    \label{tab:snb-workloads}
    \vspace{-2.5ex}
\end{table}

